Fantastic Gains and Where to Find Them: On the Existence and Prospect of General Knowledge Transfer between Any Pretrained Model

Training deep networks requires various design decisions regarding for instance their architecture, data augmentation, or optimization. In this work, we find these training variations to result in networks learning unique feature sets from the data. Using public model libraries comprising thousands of models trained on canonical datasets like ImageNet, we observe that for arbitrary pairings of pretrained models, one model extracts significant data context unavailable in the other -- independent of overall performance. Given any arbitrary pairing of pretrained models and no external rankings (such as separate test sets, e.g. due to data privacy), we investigate if it is possible to transfer such "complementary" knowledge from one model to another without performance degradation -- a task made particularly difficult as additional knowledge can be contained in stronger, equiperformant or weaker models. Yet facilitating robust transfer in scenarios agnostic to pretrained model pairings would unlock auxiliary gains and knowledge fusion from any model repository without restrictions on model and problem specifics - including from weaker, lower-performance models. This work therefore provides an initial, in-depth exploration on the viability of such general-purpose knowledge transfer. Across large-scale experiments, we first reveal the shortcomings of standard knowledge distillation techniques, and then propose a much more general extension through data partitioning for successful transfer between nearly all pretrained models, which we show can also be done unsupervised. Finally, we assess both the scalability and impact of fundamental model properties on successful model-agnostic knowledge transfer.

==> broader_impact.tex <==
\section{Broader Impact}
\label{sec:broader_impact}


==> latex_figures/prediction_flips_similarities.tex <==
\begin{wrapfigure}{r}{0.48\linewidth}
    \centering
    %\fbox{
    \includegraphics[width=\linewidth]{figures/prediction_flips_sim_plot.pdf}
    %}
    \vspace{-5pt}
    \caption{Average semantic similarity between class labels of the classes with the highest percentage of positive prediction flips, reported as the relative difference to the average similarity among all classes.}
    \label{fig:prediction_flips_similarities}
    \vspace{-10pt}    
\end{wrapfigure}

==> latex_figures/student_feats.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/student_feature_influence.pdf}
    \caption{Analysis on the impact of the sutdent model's a) performance, b) size, and c) architecture on the distillation delta. Each marker represents one student model. In each subplot we connect the student models for which the two remaining model features are similar.}
    \label{fig:student_features}
\end{figure}

==> tables/dist_deltas_full_imagenet_new.tex <==
\begin{table}[t]
\caption{Knowledge Transfer results on full ImageNet, from four teacher to eight selected student models (see Sup.). We group the teacher-student pairs by their performance difference $\Delta_\text{acc}$ and report the mean and std of the transfer delta $\Delta_\text{tansf.}$ for each group. The results provide further evidence that a continual learning treatment of the transfer problem allows for more consistent knowledge transfer across arbitrary student/teacher model pairs.}
\centering
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{l|cc}
    \toprule
    $\Delta_\text{acc}$ & $\Delta_\text{transf.}$ KL-Dist. & $\Delta_\text{transf.}$ KL+DP Dist. \\
    \midrule
    (-15, -3] & -0.87 ($\pm$ 0.37) & \textbf{0.23} ($\pm$ 0.14) \\
    (-3, -1] & -0.33 ($\pm$ 0.16) & \textbf{0.26} ($\pm$ 0.12) \\
    (-1, 1] & -0.06 ($\pm$ 0.43) & \textbf{0.31} ($\pm$ 0.16) \\
    (1, 3] & \textbf{0.63} ($\pm$ 0.48) & 0.54 ($\pm$ 0.30) \\
    (3, 15] & 0.38 ($\pm$ 0.21) & \textbf{0.40} ($\pm$ 0.18) \\
    \midrule
    \multicolumn{4}{r|}{\textbf{Avg. Rank}} & 1.8 & \textbf{1.2}\\
    \bottomrule
\end{tabular}}
\label{tab:imagenet_dist_deltas}
\vspace{-5pt}
\end{table}

==> tables/sup_v_unsup.tex <==
\begin{wraptable}{r}{0.5\linewidth}
\vspace{-10pt}
\caption{\textit{Comparison between supervised and unsupervised KL+DP distillation on ImageNet} for eight selected students and four teachers, respectively. Results show that fully unsupervised knowledge transfer between experts is not only possible but can even outperform supervised transfer.}
\label{tab:imagenet_supervised_unsupervised_MT}
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{lcc}
    \toprule
    \multirow{2}{*}{\textbf{Students}} & $\Delta_\text{transf.}$ KL+DP & $\Delta_\text{transf.}$ KL+DP \\
     & \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{Unsupervised} \\
    \midrule
    XCiT-P16 \cite{elnouby2021xcit} &  0.65 ($\pm$0.26) & \textbf{0.96} ($\pm$0.42) \\
    PiT-B \cite{heo2021pit} &  0.55 ($\pm$0.25) & \textbf{0.95} ($\pm$0.52) \\
    PiT-XS \cite{heo2021pit} &  \textbf{0.40} ($\pm$0.12) & 0.35 ($\pm$0.18) \\
    \midrule
    SeNet154 \cite{he2018gluon} & \textbf{0.27} ($\pm$0.17) & 0.25 ($\pm$0.15)\\
    ConvNext \cite{liu2022convnet} & \textbf{0.33} ($\pm$0.14) & 0.28 ($\pm$0.14) \\
    ResNetV2 \cite{he2016resnetv2} & \textbf{0.23} ($\pm$0.08) & \textbf{0.23} ($\pm$0.09)\\
    \midrule
    % Mixer-L16 (*) \cite{tolstikhin2021mlpmixer} & MLP &  72.07 & 208.20 & \textbf{7.02} ($\pm$0.17) &  5.45 ($\pm$0.27) \\
    Mixer-B16 \cite{tolstikhin2021mlpmixer} & 0.15 ($\pm$0.13) & \textbf{0.17} ($\pm$0.15)\\
    ResMLP-24 \cite{touvron2021resmlp} &  \textbf{0.33} ($\pm$0.19) & 0.29 ($\pm$0.24) \\
    % ResMLP-12 \cite{touvron2021resmlp} & \textbf{0.39} ($\pm$0.11) & \textbf{0.35} ($\pm$0.38) \\
    \bottomrule
\end{tabular}}
\end{wraptable}
